Esports World Model Dataset

Interactive world models must capture how multiple participants jointly change a shared environment while observing different parts of it. Competitive games make this challenge concrete: players cooperate and compete, while fog of war, team vision and camera placement determine what each can see. Modeling these interactions requires data that connect individual observations and actions to shared state and events. We introduce the Esports World Model Dataset (EWM), a collection of human gameplay spanning StarCraft II, Dota 2 and Counter-Strike 2, with 3,053 games and maps and approximately 4,880 player-view hours, including estimated hours for the ongoing CS2 extension. It includes 4,628 completed StarCraft II views, all ten perspectives for 303 Dota 2 matches, and up to ten views per round in CS2. Across these views, replay-clock alignment connects rendered video with game-native actions, structured state and events from the same match. The three games expose complementary observation conditions: private fog of war, shared team vision and first-person viewpoints. In StarCraft II, player-specific entity records further distinguish live observations from remembered snapshots and link co-observed entities across opposing views. Together with temporal alignment, these records allow researchers to distinguish legitimate information differences from disagreement about shared state. By connecting human decisions, shared dynamics and player-specific information, EWM supports research toward jointly controlled multiplayer world models and interactive environments populated by teammates and opponents learned from human play.

==> figures/incoming_20261010/records/cs2_action_rec.tex <==
// events.parquet, tick 132117
{
  "tick": 132117,
  "event_type": "kill",
  "attacker_name": "FalleN",
  "attacker_steamid": "76561197960690195",
  "user_name": "donk",
  "user_steamid": "76561198386265483",
  "weapon": "hkp2000",
  "hitgroup": "chest",
  "headshot": false,
  "distance": 7.1,
  "dmg_health": 16.0,
  "dmg_armor": 8.0,
  "penetrated": 0.0,
  "thrusmoke": false,
  "attackerblind": false
}


==> figures/incoming_20261010/records/cs2_state_rec.tex <==
// 76561197960690195/state.parquet, tick 132100
{
  "tick": 132100,
  "name": "FalleN",
  "team_name": "CT",
  "X": 322.28,
  "Y": -826.39,
  "Z": -127.97,
  "velocity_X": 31.51,
  "velocity_Y": 50.26,
  "yaw": -32.92,
  "pitch": 70.92,
  "health": 95,
  "armor_value": 0,
  "active_weapon_name": "P2000",
  "active_weapon_ammo": 12.0,
  "balance": 1600,
  "is_alive": true,
  "FORWARD": false,
  "BACK": false,
  "LEFT": true,
  "RIGHT": true,
  "FIRE": false,
  "DUCK": false,
  "JUMP": false,
  "buttons": 1536
}


==> figures/records/cs2_action_compact_rec.tex <==
// events.parquet, tick 132372
{
  "tick": 132372, "event_type": "kill",
  "attacker_name": "tN1R",
  "attacker_steamid": "76561198872013168",
  "user_name": "YEKINDAR",
  "user_steamid": "76561198134401925",
  "weapon": "mac10", "hitgroup": "chest",
  "headshot": false, "distance": 5.64,
  "dmg_health": 26.0, "dmg_armor": 0.0,
  "penetrated": 0.0, "thrusmoke": false,
  "attackerblind": false
}


==> figures/records/cs2_state_compact_rec.tex <==
// 76561198872013168/state.parquet, tick 132356
{
  "tick": 132356, "name": "tN1R",
  "team_name": "TERRORIST", "X": 391.01, "Y": -912.46,
  "Z": -391.47, "velocity_X": 67.02,
  "velocity_Y": 187.63, "yaw": 5.21, "pitch": 7.92,
  "health": 68, "armor_value": 86,
  "active_weapon_name": "MAC-10",
  "active_weapon_ammo": 8.0, "balance": 250,
  "is_alive": true, "FORWARD": false, "BACK": false,
  "LEFT": true, "RIGHT": false, "FIRE": false,
  "DUCK": false, "JUMP": false, "buttons": 512
}


==> figures/records/dota_action_compact_rec.tex <==
// messages.parquet, tick 85916: unit order (entity 9 = slot 8)
{
  "tick": 85916,
  "type": "DOTA_UM_SpectatorPlayerUnitOrders",
  "payload": {
    "entindex": 9, "orderType": 4, "units": [461],
    "targetIndex": 1383, "abilityId": -1,
    "queue": false, "sequenceNumber": 10299
  }
}

// messages.parquet, tick 85916: hero kill
{
  "tick": 85916, "type": "DOTA_UM_ChatEvent",
  "payload": {
    "type": "CHAT_MESSAGE_HERO_KILL", "value": 456,
    "playerid_1": 4, "playerid_2": 5, "value2": 585,
    "time": 2062.63
  }
}


==> figures/records/dota_state_compact_rec.tex <==
// messages.parquet, tick 85916: combat log
{
  "tick": 85916, "type": "DOTA_UM_CombatLogDataHltv",
  "payload": {
    "type": "DOTA_COMBATLOG_DEATH", "attackerName": 9,
    "targetName": 7, "attackerTeam": 3,
    "targetTeam": 2, "isAttackerHero": true,
    "isTargetHero": true, "value": 1335,
    "timestamp": 2873.0
  }
}

// slot04/alignment.parquet: the frame at tick 85916
{
  "player_slot": 4, "global_frame_index": 64884,
  "global_video_time_s": 2162.8, "replay_tick": 85916,
  "action_count_player": 2
}

// slot05/alignment.parquet: the frame at tick 85916
{
  "player_slot": 5, "global_frame_index": 64886,
  "global_video_time_s": 2162.87, "replay_tick": 85916,
  "action_count_player": 0
}


==> figures/records/sc2_action_compact_rec.tex <==
// Player 1 trajectory, action at game loop 12048
{
  "game_loop": 12048,
  "action": [
    {
      "game_loop": 12048, "type": "unit_command",
      "ability_id": 23.0,
      "unit_tags": "[28 unit tags]",
      "queue_command": false, "target_unit_tag": null,
      "target_world_pos": {"x": 61.47, "y": 113.29},
      "camera_world_pos": null
    }
  ]
}

// Player 1 trajectory, step 12056
{
  "view_id": "sc2_5fb15bea5b7c1a55769131f5.p0",
  "step_index": 12056, "game_loop": 12057,
  "timestamp_s": 538.26, "rgb_frame_index": 12056,
  "minimap_frame_index": 12056,
  "observation": {
    "camera": {"x": 52.73, "y": 103.63},
    "resources": {
      "minerals": 305, "vespene": 319,
      "food_used": 137, "food_cap": 149,
      "food_army": 80
    },
    "units": "[318 unit records]"
  }
}


==> figures/records/sc2_state_compact_rec.tex <==
// Player 1 (owner): unit 4392747010 at game loop 12057
{
  "tag": 4392747010, "unit_type": 141, "owner": 1,
  "alliance": 1, "display_type": 1,
  "pos": {"x": 47.36, "y": 104.26, "z": 11.99},
  "health": 10.0, "shield": 350.0, "energy": 0.0,
  "orders": [
    {
      "ability_id": 23, "progress": 0.0,
      "target_unit_tag": 4384096265.0,
      "target_world_pos": null
    },
    {
      "ability_id": 23, "progress": 0.0,
      "target_unit_tag": null,
      "target_world_pos": {"x": 61.47, "y": 113.29}
    }
  ]
}

// Player 2 (opponent): the same unit at the same game loop
{
  "tag": 4392747010, "unit_type": 141, "owner": 1,
  "alliance": 4, "display_type": 1,
  "pos": {"x": 47.36, "y": 104.26, "z": 11.99},
  "health": 10.0, "shield": 350.0, "energy": 0.0,
  "orders": []
}

